Cloaking the Clock: Emulating Clock Skew in Controller Area Networks

Automobiles are equipped with Electronic Control Units (ECU) that communicate via in-vehicle network protocol standards such as Controller Area Network (CAN). These protocols are designed under the assumption that separating in-vehicle communications from external networks is sufficient for protection against cyber attacks. This assumption, however, has been shown to be invalid by recent attacks in which adversaries were able to infiltrate the in-vehicle network. Motivated by these attacks, intrusion detection systems (IDSs) have been proposed for in-vehicle networks that attempt to detect attacks by making use of device fingerprinting using properties such as clock skew of an ECU. In this paper, we propose the cloaking attack, an intelligent masquerade attack in which an adversary modifies the timing of transmitted messages in order to match the clock skew of a targeted ECU. The attack leverages the fact that, while the clock skew is a physical property of each ECU that cannot be changed by the adversary, the estimation of the clock skew by other ECUs is based on network traffic, which, being a cyber component only, can be modified by an adversary. We implement the proposed cloaking attack and test it on two IDSs, namely, the current state-of-the-art IDS and a new IDS that we develop based on the widely-used Network Time Protocol (NTP). We implement the cloaking attack on two hardware testbeds, a prototype and a real connected vehicle, and show that it can always deceive both IDSs. We also introduce a new metric called the Maximum Slackness Index to quantify the effectiveness of the cloaking attack even when the adversary is unable to precisely match the clock skew of the targeted ECU.

==> sections/evaluation.tex <==
\section{Evaluation}
\label{sec:evaluation}
In this section, we conduct extensive experiments to evaluate the performance of the proposed cloaking attack on two CAN bus testbeds, and demonstrate that the cloaking attack is able to bypass both the Cho-Shin CIDS and the NTP-based CIDS. 

\subsection{Testbeds}
We built two CAN bus testbeds: a CAN bus prototype and a CAN tested based on a real vehicle (University of Washington (UW) EcoCar\footnote{The EcoCar was originally a 2016 Cherolet Camaro donated by General Motors as part of a competition.
	Researchers at UW later converted into a hybrid electric vehicle to develop next-generation vehicle technologies. } \cite{ecocar}).
Compared with the prototype with $3$ ECUs, the EcoCar testbed has \cmt{$8$} stock ECUs and one added by researchers.
There are a total of $89$ messages with different IDs, and at least $2500$ messages are transmitted every second. 
Hence, the prototype is ideal for prototyping, whereas the EcoCar testbed provides a real CAN environment to evaluate and demonstrate the proposed cloaking attack. 

\begin{figure}[ht!]
	\centering
	\begin{subfigure}[h]{0.43\columnwidth} % {0.48\columnwidth}
		\includegraphics[width=\columnwidth]{./figures/new_figs/arduino_testbed}
		\caption{CAN bus prototype}
		\label{fig:arduino_testbed}
	\end{subfigure}
	\begin{subfigure}[h]{0.55\columnwidth} % {0.48\columnwidth}
		\includegraphics[width=\columnwidth]{./figures/new_figs/real_vehicle_testbed}
		\caption{EcoCar testbed}
		\label{fig:real_vehicle_testbed}
	\end{subfigure}
	\caption{CAN testbeds. The CAN bus prototype is connected to the CAN bus inside the EcoCar via the OBD-II port to build the EcoCar testbed.  }
\end{figure}

\subsubsection{CAN Bus Prototype}

% Testbed and data collection
As shown in Fig.~\ref{fig:arduino_testbed}, our CAN bus prototype consists of three ECUs.
Each ECU is composed of an Arduino UNO board and a Sparkfun CAN bus shield.
%
%Arduino UNO board creates the contents of a CAN message and determines the period of a message.
%
%Sparkfun CAN bus shield constructs a CAN message using data from Arduino UNO board, and decodes a CAN message.
%
The CAN bus shield uses a Microchip MCP2515 CAN controller, a Microchip MCP2551 CAN transceiver, and a 120$\Omega$ terminator resistor. 
%
The baud rate of the prototype is set to $500$Kbps as in typical  CAN buses.
%
ECU $1$ is the receiving ECU that implements the CIDS.
%
ECU $2$ is the legitimate ECU (the weak attacker) that transmits messages 0x11 every $100$ms (i.e., $10$Hz).
ECU $3$ is the strong attacker that aims to impersonate ECU $2$ in a masquerade or cloaking attack.


\subsubsection{EcoCar CAN testbed}
As shown in Fig. \ref{fig:real_vehicle_testbed}, the CAN bus prototype is connected to the in-vehicle CAN bus of the EcoCar via the On-Board Diagnostics (OBD-II)  port to build the EcoCar testbed. 
During our experiments, the EcoCar is in park mode in an isolated and controlled environment, but all ECUs are functional and actively exchange CAN messages.

Due to the large CAN traffic and limited computing capability, the Arduino-based ECU is not able to capture all messages. 
Hence, we build a fourth ECU that consists of a Raspberry Pi 3 and a PiCAN 2 board (using the same CAN controller and transceiver as in the CAN bus shield) as the receiving ECU. 
A stock ECU is considered as the legitimate ECU (the weak attacker) which transmits message 0x184 every $100$ms (i.e., $10$Hz), and the same Arduino-based ECU $3$ is used as the strong attacker that injects spoofed messages.


%\subsubsection{CAN Log Data}
%
%Ruth \emph{et. al.} provide CAN traffic data logged from a Toyota Camry 2010, and the data is logged through a Gryphon S3 and Hercules software \cite{Ruth:2012:Accuracy}.
%
%They ran 14 independent experiments, and each experiment is about 4 minutes long.
%
%In Toyota Camry 2010, there are 42 distinct messages transmitted on the CAN bus.

%Table \ref{table:parameter_CIDS} summarizes the values of $N$, $\gamma$, and $\kappa$ that guarantee zero false-positive probability by CUSUM.

% Table: Parameter setting
%\begin{table}[b!]
%	\caption {Values of $N$, $\gamma$, and $\kappa$ are summarized depending on the types of CIDS and CAN system (i.e., CAN testbed and Ecocar.).}
%	\label{table:parameter_CIDS}
%	\begin{center}
%		\resizebox{0.45\textwidth}{!}
%		{
%			\begin{tabular}{|c|c|c|c|c|}
%				\hline
%				\multirow{2}{*}{Parameters} & \multicolumn{2}{c|}{Cho-Shin CIDS} &
%				\multicolumn{2}{c|}{NTP-based CIDS} \\
%				\cline{2-5}
%				& CAN testbed & Ecocar & CAN testbed & Ecocar  \\
%				\hline
%				N & 20 & 20 & 20 & 20 \\
%				\hline
%				$\gamma$ & 3 & 3 & 4 & 4 \\
%				\hline
%				$\kappa$ & 5 & 8 & 5 & 8 \\
%				\hline
%			\end{tabular}
%		}
%	\end{center}
%\end{table}


%The receiver, denoted as ECU R, receives all messages in the CAN bus and records receive timestamps of each message according to its local clock.

%
%Ecocar has an operating CAN bus with legitimate ECUs, and these ECUs transmit periodic messages.
%
%We connect the testbed ECU to Ecocar through OBD-II port, and inject attack messages as well as collect messages for analysis.
%
%Arduino UNO board can only record 10 messages per second accurately and there are 2400 messages per second in Ecocar.
%
%Hence, we build two sets of testbed ECUs which is composed of Raspberry Pi 3 and PiCAN2 Duo CAN-Bus Board, because the clock speed of Raspberry Pi 3 is 1.2GHz whereas that of Arduino UNO is 1.6MHz.
%
%We use the testbed ECUs with Raspberry Pi 3 for data collection at Ecocar and mount the cloaking attack on the correlation detector because receiving and filtering the target message is essential step of the cloaking attack on the correlation detector.

%\begin{figure*}
%	\centering
%	\begin{subfigure}[b]{0.3\textwidth}
%		\includegraphics[width=\textwidth]{./figures/toyota_counter_example_starting_index.eps}
%		\caption{Starting index is 2.}
%		\label{fig:counter_example:startingIndex}
%	\end{subfigure}
%	\begin{subfigure}[b]{0.3\textwidth}
%		\includegraphics[width=\textwidth]{./figures/toyota_counter_example_N30.eps}
%		\caption{Number of messages in a batch is 30.}
%		\label{fig:counter_example:differentN}
%	\end{subfigure}
%	\begin{subfigure}[b]{0.3\textwidth}
%		\includegraphics[width=\textwidth]{./figures/toyota_accoffset_run32_shin.eps}
%		\caption{Run 32}
%		\label{fig:counter_example:run32}
%	\end{subfigure}
%	\caption{Examples show that clock skew of one ECU changes for different setting in Cho-Shin CIDS using data of Toyota Camry 2010.
		%
%		Fig. \ref{fig:counter_example:startingIndex} shows that slopes of messages 0x223 and 0x224 swap each other as we change the starting index of the input data from 1 to 2.
		%
%		Fig. \ref{fig:counter_example:differentN} shows that clock skew of message 0x020 changes from 273ppm to 151ppm as the number of messages in a batch is changed from 20 to 30.
		%
%		Comparing Fig. \ref{fig:toyota_accoffset_shin:run25} and Fig. \ref{fig:counter_example:run32}, the clock skew of message 0x020 in Run 25 is 273ppm whereas that in Run 32 is 306ppm.}
%	\label{fig:counter_example}
%\end{figure*}

%We observed that a clock skew of an ECU that is computed by Cho-Shin CIDS is not consistent as changing the starting indices of input data, the number of messages in a batch, and experiment sets.
%
%Comparing Figs. \ref{fig:toyota_accoffset_shin:run25} and \ref{fig:counter_example:startingIndex}, the slopes of messages 0x223 and 0x224 swap each other as changing the start index of input data.
%
%Comparing Figs. \ref{fig:toyota_accoffset_shin:run25} and \ref{fig:counter_example:differentN}, the clock skew of message 0x020 changes from 273ppm to 151ppm as changing $N$ from 20 to 30.
%
%Comparing Figs. \ref{fig:toyota_accoffset_shin:run25} and \ref{fig:counter_example:run32}, the clock skew of message 0x020 different between two experiment sets.
%
%Hence, the clock skew of one ECU is not constant which indicates that the clock skew is not exploited to identify ECUs in Cho-Shin CIDS.
%
%However, average offset in the CIDS is essentially a measure of difference in inter-arrival time between the previous and current batch.
%
%When the masquerade attack occurs, the inter-arrival time (i.e., the measured period) of ECU A's messages is very different from the that of ECU B's messages, since the clock skew is different.
%
%Thus, Cho-Shin CIDS still can detect the masquerade attack by capturing abrupt changes in the inter-arrival time.
%
%The fact that Cho-Shin CIDS does not exploit clock skew as a fingerprint of ECU leads us to propose a new CIDS, called NTP-based CIDS, which indeeds captures clock skew in order to identify each ECU.

%Now we verify that NTP-based CIDS indeeds captures clock skew of an ECU for ECU identification based on the first and second order statistics of clock skew as changing starting index of input data, number of messages in a batch, and experiments using Toyota Camry 2010 data.
%
%The computed clock skew is more consistent as the standard deviation of clock skew becomes smaller.
%
%Table \ref{table:statistics_index} shows that the clock skew computed by NTP-based CIDS is consistent as the starting index changes.
%
%Table \ref{table:statistics_N} shows that the clock skew computed by NTP-based CIDS is consistent as the number of messages per batch changes.
%
%Ruth provides CAN raw data for many experiment sets using Toyota Camry 2010. We select 14 experiments sets.
%
%Table \ref{table:statistics_experiment} shows that the clock skew computed by NTP-based CIDS is consistent for different experiments.
%
%The standard deviation of clock skew computed by Cho-Shin CIDS is always larger than that by NTP-based CIDS for the same message.
%
%In addition, the maximum standard deviation of clock skew computed by NTP-based CIDS is 1.7820 which indicates that the values of clock skew deviates by 1.7820ppm at most.
%
%Hence, we verify that the NTP-based CIDS exploits clock skew to identify ECUs in CAN bus.

% Table: starting index
%\begin{table}[h]
%	\caption {Comparison on the first and second order statistics of clock skew computed by Cho-Shin and NTP-based CIDSs as the starting index changes from 1 to 19 using Toyota Camry 2010 data. Unit is in ppm.} \label{table:statistics_index}
%	\begin{center}
%		\resizebox{0.45\textwidth}{!}
%		{
%		\begin{tabular}{|c|c|c|c|c|}
%			\hline
%			\multirow{2}{*}{Message ID} & \multicolumn{2}{c|}{Cho-Shin CIDS} &
%			\multicolumn{2}{c|}{NTP-based CIDS} \\
%			\cline{2-5}
%			& Mean & \begin{tabular}{@{}c@{}}Standard \\ Deviation\end{tabular} & Mean & \begin{tabular}{@{}c@{}}Standard \\ Deviation\end{tabular}  \\
%			\hline
%			0x020 & 293.26 & 12.0980 & 167.71 & 0.2405 \\
%			\hline
%			0x0B2 & 296.75 & 11.8072 & 167.70 & 0.2396 \\
%			\hline
%			0x223 & 109.73 & 16.1452 & 167.85 & 0.3346 \\
%			\hline
%			0x224 & 108.90 & 16.9995 & 167.97 & 0.4822 \\
%			\hline
%		\end{tabular}
%		}
%	\end{center}
%\end{table}

% Table: Number of messages in a batch
%\begin{table}[h]
%	\caption {Comparison on the first and second order statistics of clock skew computed by Cho-Shin and NTP-based CIDSs as the number of messages changes from 20 to 100 by step size of 20 using Toyota Camry 2010 data. Unit is in ppm.} \label{table:statistics_N}
%	\begin{center}
%		\resizebox{0.45\textwidth}{!}
%		{
%			\begin{tabular}{|c|c|c|c|c|}
%				\hline
%				\multirow{2}{*}{Message ID} & \multicolumn{2}{c|}{Cho-Shin CIDS} &
%				\multicolumn{2}{c|}{NTP-based CIDS} \\
%				\cline{2-5}
%				& Mean & \begin{tabular}{@{}c@{}}Standard \\ Deviation\end{tabular} & Mean & \begin{tabular}{@{}c@{}}Standard \\ Deviation\end{tabular}  \\
%				\hline
%				0x020 & 115.57 & 92.3658 & 167.65 & 0.3533 \\
%				\hline
%				0x0B2 & 118.38 & 94.4385 & 167.66 & 0.4006 \\
%				\hline
%				0x223 & 63.37 & 41.7845 & 167.44 & 0.2292 \\
%				\hline
%				0x224 & 44.83 & 29.0912 & 167.60 & 0.8678 \\
%				\hline
%			\end{tabular}
%		}
%	\end{center}
%\end{table}

% Table: Experiments (run files)
%\begin{table}[h]
%	\caption {Comparison on the first and second order statistics of clock skew computed by Cho-Shin and NTP-based CIDSs for 14 different experiment sets using Toyota Camry 2010 data. Unit is in ppm.} \label{table:statistics_experiment}
%	\begin{center}
%		\resizebox{0.45\textwidth}{!}
%		{
%			\begin{tabular}{|c|c|c|c|c|}
%				\hline
%				\multirow{2}{*}{Message ID} & \multicolumn{2}{c|}{Cho-Shin CIDS} &
%				\multicolumn{2}{c|}{NTP-based CIDS} \\
%				\cline{2-5}
%				& Mean & \begin{tabular}{@{}c@{}}Standard \\ Deviation\end{tabular} & Mean & \begin{tabular}{@{}c@{}}Standard \\ Deviation\end{tabular}  \\
%				\hline
%				0x020 & 290.81 & 20.1015 & 167.36 & 1.3162 \\
%				\hline
%				0x0B2 & 293.08 & 19.3584 & 167.35 & 1.3752 \\
%				\hline
%				0x223 & 124.95 & 25.3284 & 166.79 & 1.7820 \\
%				\hline
%				0x224 & 120.98 & 32.6015 & 167.80 & 1.7358 \\
%				\hline
%			\end{tabular}
%		}
%	\end{center}
%\end{table}

% Arduino Example
\begin{figure}[t!]
	\centering
	\begin{subfigure}[h]{0.49\columnwidth} % {0.48\columnwidth}
		\captionsetup{justification=centering}
		\includegraphics[width=\columnwidth]{./figures/arduino_example_ntp_avg_offset_combined.eps}
		\caption{Average offset}
		\label{fig:arduino_avg_offset}
	\end{subfigure}
	\begin{subfigure}[h]{0.49\columnwidth} % {0.48\columnwidth}
		\captionsetup{justification=centering}
		\includegraphics[width=\columnwidth]{./figures/arduino_example_ntp_acc_offset_combined.eps}
		\caption{Accumulated offset}
		\label{fig:arduino_acc_offset}
	\end{subfigure}
	\\
	\begin{subfigure}[h]{0.49\columnwidth} % {0.48\columnwidth}
		\captionsetup{justification=centering}
		\includegraphics[width=\columnwidth]{./figures/arduino_example_naive_attack_ntp_control_limit.eps}
		\caption{Control limits under the masquerade attack}
		\label{fig:arduino_control_limit_masquerade}
	\end{subfigure}
	\begin{subfigure}[h]{0.49\columnwidth} % {0.48\columnwidth}
		\captionsetup{justification=centering}
		\includegraphics[width=\columnwidth]{./figures/arduino_example_cloaking_attack_ntp_control_limit.eps}
		\caption{Control limits under the cloaking attack}
		\label{fig:arduino_control_limit_cloaking}
	\end{subfigure}
	\caption{Behavior of the NTP-based CIDS under the masquerade and cloaking attacks on the CAN bus prototype, in terms of average offset, accumulated offset and control limits.}
	\label{fig:arduino_one_experiment_example}
\end{figure}


\subsection{Example of NTP-based CIDS}\label{sec:evaluation_example}
First of all, we would like to understand the behavior of the NTP-based CIDS under the masquerade attack, and check if it can detect the intrusion under the cloaking attack. 
In the example, we set ... \cmt{CIDS parameters}
As shown in Fig. \ref{fig:masquerade_attack_model}, the CIDS first tracks the clock skew of message 0x11 from the legitimate ECU for $1000$ seconds, before the attack happens. 
Then the CIDS is fed with the timestamps of attack messages.
For the masquerade attack, the strong attacker transmits every $T=100$ms as per its local clock. 
For the cloaking attack, the strong attacker observes the inter-arrival time of message 0x11 to around \cmt{???}, and it adjusts the message inter-departure time to be $\tilde{T}=100039\mu$s, where $\Delta T = 39\mu$s.
\cmt{The time resolution of CAN bus is $4\mu$s, how did you manage to get the $39\mu$s?}

As shown in Fig. \ref{fig:arduino_one_experiment_example}, when the masquerading attack happens, the average offset immediately jumps from around $-11\mu$s to around $28\mu$s (Fig. \ref{fig:arduino_avg_offset}), and the slope changes from $-118.9$ppm to $275.3$ppm (Fig. \ref{fig:arduino_acc_offset}), because of the very distinct clock skews between legitimate and masquerading ECUs. 
As a result, such deviations add up and cause the control limits of the CIDS to explode (Fig.~\ref{fig:arduino_control_limit_masquerade}).
In contrast, under the cloaking attack, the average offset stays almost the same as the original curve.
The slope of 
does the accumulated offset. 
Since the deviations are so small, control limits are always zero, and thus the CIDS is not able to detect the cloaking attack (Fig.~\ref{fig:arduino_control_limit_cloaking}).
We do not include an example from the EcoCar tested, since it provides very similar observations. 
%Details about the behavior of the Cho-Shin CIDS are available in \cite{Shin:2016:finger}.

%On the EcoCar CAN testbed, the strong attacker injects the message 0x180 with the added delay of -28$\mu s$ in order to attack the message 0x184.


\subsection{Performance of Cloaking Attack on Clock Skew Detector}

% Ecocar Example
%\begin{figure}
%	\centering
%	\begin{subfigure}[b]{0.49\columnwidth} % {0.48\columnwidth}
%		\includegraphics[width=\columnwidth]{./figures/ecocar_example_ntp_avg_offset_combined.eps}
%		\caption{Average offset}
%		\label{fig:ecocar_avg_offset}
%	\end{subfigure}
%	\begin{subfigure}[b]{0.49\columnwidth} % {0.48\columnwidth}
%		\includegraphics[width=\columnwidth]{./figures/ecocar_example_ntp_acc_offset_combined.eps}
%		\caption{Accumulated offset}
%		\label{fig:ecocar_acc_offset}
%	\end{subfigure}
%	\\
%	\begin{subfigure}[b]{0.49\columnwidth} % {0.48\columnwidth}
%		\includegraphics[width=\columnwidth]{./figures/ecocar_example_naive_attack_ntp_control_limit.eps}
%		\caption{Control limits of masquerade attack}
%		\label{fig:ecocar_control_limit_masquerade}
%	\end{subfigure}
%	\begin{subfigure}[b]{0.49\columnwidth} % {0.48\columnwidth}
%		\includegraphics[width=\columnwidth]{./figures/ecocar_example_cloaking_attack_ntp_control_limit.eps}
%		\caption{Control limits of cloaking attack}
%		\label{fig:ecocar_control_limit_cloaking}
%	\end{subfigure}
%	\caption{Comparison of masquerade and cloaking attacks on UW Ecocar with respect to various metrics.}
%	\label{fig:ecocar_one_experiment_example}
%\end{figure}

% Successful Rates
\begin{figure}[t!]
	\centering
	\begin{subfigure}[h]{0.49\columnwidth} % {0.48\columnwidth}
		\captionsetup{justification=centering}
		\captionsetup{justification=centering}
		\includegraphics[width=\columnwidth]{./figures/arduino_clock_skew_attack_rates_ChoShin_CIDS.eps}
		\caption{CAN bus prototype with the Cho-Shin CIDS}
		\label{fig:arduino_clock_skew_attack_success_rate_Cho}
	\end{subfigure}
	\begin{subfigure}[h]{0.49\columnwidth} % {0.48\columnwidth}
		\captionsetup{justification=centering}
		\includegraphics[width=\columnwidth]{./figures/ecocar_clock_skew_attack_rates_ChoShin_CIDS.eps}
		\caption{EcoCar CAN testbed with the Cho-Shin CIDS}
		\label{fig:ecocar_clock_skew_attack_success_rate_Cho}
	\end{subfigure}
	\\
	\begin{subfigure}[h]{0.49\columnwidth} % {0.48\columnwidth}
		\captionsetup{justification=centering}
		\includegraphics[width=\columnwidth]{./figures/arduino_clock_skew_attack_rates_ntp_CIDS.eps}
		\caption{CAN bus prototype with the NTP-based CIDS}
		\label{fig:arduino_clock_skew_attack_success_rate_ntp}
	\end{subfigure}
	\begin{subfigure}[h]{0.49\columnwidth} % {0.48\columnwidth}
		\captionsetup{justification=centering}
		\includegraphics[width=\columnwidth]{./figures/ecocar_clock_skew_attack_rates_ntp_CIDS.eps}
		\caption{EcoCar CAN testbed with the NTP-based CIDS}
		\label{fig:ecocar_clock_skew_attack_success_rate_ntp}
	\end{subfigure}
	\caption{Successful attack probability on the clock skew detector of the Cho-Shin CIDS and the NTP-based CIDS using the CAN bus prototype and EcoCar CAN testbed for different $n_{attack}$.}
	\label{fig:clock_skew_attack_success_rate}
\end{figure}

%For evaluation of the cloaking attack on the CAN bus prototype, ECUs A and B are considered to have been compromised as strong and weak attacker as Fig. \ref{fig:masquerade_attack_model}.
%
% ECU B initially transmits the message 0x011, and ECU A launches the cloaking attack on ECU B at $t_{attack}$=100 seconds by injecting the message 0x021, i.e., transmission of the message 0x011 is suspended.


To launch the cloaking attack, the impersonating ECU needs to transmit every $100039\mu$s on the CAN bus prototype to spoof the $10$Hz message 0x11, and every $99972\mu$s to spoof the $10$Hz message 0x184 on the EcoCar testbed.
A total of \cmt{?}-hr and \cmt{?}-hr attack data was collected from the CAN bus prototype and the EcoCar testbed, respectively, and processed offline to simulate the cloaking attack. 
Similar to the example in Section~\ref{sec:evaluation_example}, in each experiment, we feed \cmt{?} batches of normal data to a CIDS, followed by $n_{attack}$ batches of attack data. 
The attack is considered successful if it bypasses the CIDS, and failed otherwise. 
We prepare $100$ non-overlapping segments of size $n_{attack}$ from the attack data to simulate $100$ independent attacks. 
To quantify the attack performance, we compute \textit{successful attack probability}, which is the percentage of experiments where the cloaking attack is successful.


We consider the Cho-Shin CIDS and the NTP-based CIDS with batch size equal to $20$.
As in \cite{Shin:2016:finger}, the update threshold $\gamma$ is set to $3$ and the detection threshold $\Gamma$ is set to $5$ for the Cho-Shin CIDS.
For the NTP-based CIDS, we use $\gamma=4$ and $\Gamma=5$. 
For data collected from the CAN bus prototype, the sensitivity parameter $\kappa$ is set to $5$ for both CIDS's, whereas it is set $8$ (less sensitive) for data collected from the EcoCar testbed to avoid false alarms. 



%On a CAN testbed, we let the weak attacker, denoted as ECU B, transmit a 10Hz periodic message as the target message, and the strong attacker, denoted as ECU A, launches the cloaking attack on the clock skew detector observing that target message.
%
%In the cloaking attack on the correlation detector, we let 5Hz periodic message of ECU B as the target message that ECU A transmits the attack message based on reception of the target message.
%
%We verify not only the cloaking attack on the CAN testbed but also on a real vehicle, and evaluate the performance of the cloaking attack on the real vehicle.
%
%For the validation of the cloaking attack on the real vehicle, we implement the cloaking attack on and collected data from University of Washington (UW) Ecocar \cite{Crain:2014:Ecocar}.

%Let $n_{attack}$ be the number of batches in one experiment.
%
%Then, we collect $100 \times n_{attack} \times N$ messages, so 100 experiments are prepared.
%
%The successful attack probability, which is the performance metric of the cloaking attack, is defined as the ratio of the number of experiments that bypass the CIDS to the total number of experiment which is 100.
%
Fig. \ref{fig:clock_skew_attack_success_rate} shows the successful attack probability of the cloaking attack on the Cho-Shin CIDS and the NTP-based CIDS using the CAN bus prototype and the EcoCar CAN testbed.
%
%The axis of Fig. \ref{fig:clock_skew_attack_success_rate} is the normalized added delay which is defined as $\frac{\Delta T}{T}$.
%
%The periods of the target messages for the CAN testbed and Ecocar are 100ms and 10ms, respectively.
%
As shown in Fig. \ref{fig:clock_skew_attack_success_rate}, the detection probability of the NTP-based CIDS is better than that of the Cho-Shin CIDS because the NTP-based CIDS detects the attack for the smaller delay added to the inter-departure time of the attack message.
%
As shown in Figs. \ref{fig:arduino_clock_skew_attack_success_rate_Cho} and \ref{fig:arduino_clock_skew_attack_success_rate_ntp}, the cloaking attack perfectly bypasses the Cho-Shin CIDS and the NTP-based CIDS when the added delay is 39${\mu s}$ which perfectly matches the inter-arrival time between the messages 0x011 and 0x021.

First, the successful attack probability decreases as the added delay becomes farther from 39${\mu s}$ because the message 0x021's inter-arrival time at ECU R deviates more from the message 0x011's inter-arrival time.
%
Second, the cloaking attack becomes more difficult to be detected when one experiment set is composed of smaller number of batches because one of the control limits has to increase greater than 5 within smaller number of samples.
%
%In the CAN bus prototype, the strong attacker transmits the attack message every 100040$\mu s$ in the experiment using the CAN testbed.
%
%As the strong attacker inaccurately estimates the inter-arrival time of the target message, the successful attack probability decreases.
%
%Moreover, the strong attacker has to estimate the inter-arrival time of the target message more accurately as $n_{\text{attack}}$ increases since the attack can be detected more easily when more number of batches are used in one experiment.
%
%However, if the strong attacker precisely control the inter-departure time of the attack message, the cloaking attack on the clock skew detector can bypass the CIDS even when $n_{\text{attack}}$ increases.

We also implement the cloaking attack on EcoCar CAN testbed so that the feasibility of the cloaking attack can be proven on a real vehicle.
%
As shown in Figs. \ref{fig:ecocar_clock_skew_attack_success_rate_Cho} and \ref{fig:ecocar_clock_skew_attack_success_rate_ntp}, the cloaking attack can bypass the Cho-Shin CIDS and the NTP-based CIDS when the added delay is -29${\mu s}$.
%
The trends of the curve is the same as that in CAN bus prototype.

\subsection{Performance of Cloaking Attack on Correlation Detector}

\begin{figure}
	\centering
	\begin{subfigure}[h]{0.48\columnwidth} % {0.48\columnwidth}
		\captionsetup{justification=centering}
		\includegraphics[width=\columnwidth]{./figures/arduino_example_correlation_attack_cho.eps}
		\caption{CAN bus prototype with the Cho-Shin CIDS}
		\label{fig:arduino_correlation_attack_example}
	\end{subfigure}
	\begin{subfigure}[h]{0.48\columnwidth} % {0.48\columnwidth}
		\captionsetup{justification=centering}
		\includegraphics[width=\columnwidth]{./figures/ecocar_example_correlation_attack_cho.eps}
		\caption{EcoCar CAN testbed with the Cho-Shin CIDS}
		\label{fig:ecocar_correlation_attack_example}
	\end{subfigure}
	\\
	\begin{subfigure}[h]{0.48\columnwidth} % {0.48\columnwidth}
		\captionsetup{justification=centering}
		\includegraphics[width=\columnwidth]{./figures/arduino_example_correlation_attack_ntp.eps}
		\caption{CAN bus prototype with the NTP-based CIDS}
		\label{fig:arduino_correlation_attack_example}
	\end{subfigure}
	\begin{subfigure}[h]{0.48\columnwidth} % {0.48\columnwidth}
		\captionsetup{justification=centering}
		\includegraphics[width=\columnwidth]{./figures/ecocar_example_correlation_attack_ntp.eps}
		\caption{EcoCar CAN testbed with the NTP-based CIDS}
		\label{fig:ecocar_correlation_attack_example}
	\end{subfigure}
	\caption{Correlation between average offsets of weak and strong attackers' messages. }
	\label{fig:correlation_attack_example}
\end{figure}

\begin{figure}[h]
	\centering
	\includegraphics[width=90mm]{./figures/correlation_attack_roc.eps}
	\caption{ROC curve for the cloaking attack on the correlation detector using CAN bus prototype and EcoCar CAN testbed.}
	\label{fig:roc_correlation_attack}
\end{figure}

%We present one instance of the cloaking attack on the correlation detector via the scatter plots of the average offsets.
% Setups
For evaluation of the cloaking attack on the CAN bus prototype, ECU A inject the message 0x021 as soon as it receives the message 0x011 which is the transmitted by ECU B every 100ms.
%
On the EcoCar CAN testbed, the strong attacker injects the message 0C0 when it receives the message 0C1 whose period is 10ms.
%
In order to draw the plots and compute the correlation coefficient, $10^{5}$ samples are used with $N$=20.
%
We also let one experiment be 50 batches long and collected the data for 100 experiments.
%
Then, we analyze how well the cloaking attack can bypass the CIDS.

Fig. \ref{fig:correlation_attack_example} visualizes the correlation between the average offsets of target message and attack message in the CAN bus prototype and the EcoCar CAN testbed when the cloaking attack is mounted.
%
As shown in Fig. \ref{fig:correlation_attack_example}, the correlation is high (i.e., correlation is greater than 0.7 for all four cases) when the cloaking attack is launched even though the target message and the attack message are transmitted from two distinct ECUs.
%

%
%In addition to the CAN testbed, the cloaking attack on the correlation detector is mounted on Ecocar, and the clock offset of the attack message can be highly correlated using the cloaking attack on the correlation detector as shown in Fig. \ref{fig:ecocar_correlation_attack_example}.
%
%(In \cite{Shin:2016:finger}, CIDS decides the two messages are transmitted from one ECU if the correlation coefficient is greater than 0.8.)

%Also, the cloaking attack on the correlation detector matches the strong attacker's clock skew to the weak attacker's clock skew as shown in \hl{Fig.}.
%
%Hence, the cloaking attack on the correlation detector is not caught by the clock skew detector as well.
%\hl{(In case, I can provide sets of figures which are avg offset, acc offset, and control limits to rigorously show that cloaking attack on correlation detector is not detected by clock skew detector.)}

%Then, we evaluate the performance of the cloaking attack on the correlation detector with respect to the successful attack probability.
%
%Each experiment is consist of 50 batches and 100 experiments are considered.
%
Fig. \ref{fig:roc_correlation_attack} shows the Receiver Operating Characteristic (ROC) curve of the Cho-Shin CIDS and the NTP-based CIDS which represents the trade off between the false-positive and detection probability when the cloaking attack on the correlation detector is mounted. 
%
For the CAN bus prototype, the successful detection probability is 0\% and 2\% when the false-positive probability is set to 0. 
%
%For the experiment on EcoCar CAN testbed, two 100Hz periodic messages which are consecutively transmitted from one ECU are selected,and the message transmitted first is chosen as the target message.
%
%Also, the attack message is transmitted as soon as the strong attacker receives the target message.
%
%The curve of the cloaking attack is close enough to that of the case where two messages are transmitted from one ECU, hence the cloaking attack on the correlation detector can be successfully mounted.

==> sections/evaluation_E.tex <==


